Verification of Component-based Systems with Recursive Architectures

We study a sound verification method for parametric component-based systems. The method uses a resource logic, a new formal specification language for distributed systems consisting of a finite yet unbounded number of components. The logic allows the description of architecture configurations coordinating instances of a finite number of types of components, by means of inductive definitions similar to the ones used to describe algebraic data types or recursive data structures. For parametric systems specified in this logic, we show that decision problems such as reaching deadlock or violating critical section are undecidable, in general. Despite this negative result, we provide for these decision problems practical semi-algorithms relying on the automatic synthesis of structural invariants allowing the proof of general safety properties. The invariants are defined using the WSkS fragment of the monadic second order logic, known to be decidable by a classical automata-logic connection, thus reducing a verification problem to checking satisfiability of a WSkS formula.

==> symmetry.tex <==
\subsection{The Symmetry of Parametric Problems}
\label{sec:symmetry}

We prove a symmetry property of the decision problems considered,
implying that the answer of a particular instance of a problem does
not depend on the particular choice of indices used to model the
system. Consider a fixed signature $\signature$, with component types
$\comps = \set{\acomp_1, \ldots, \acomp_\ncomps}$ and interaction
types $\interacs = \set{\ainterac_1, \ldots, \ainterac_\ninteracs}$,
and a behavior map $\beh$, in the rest of this section. Given an
architecture $\struc$ over $\signature$ and a tuple of bijections
$\vec{f} = \tuple{f_1, \ldots, f_\ncomps} : \universe \rightarrow
\universe$, one for each component type, we define:
\[\begin{array}{rcl}
\hspace*{-2mm}(\vec{f}(\struc))(\acomp_i) & \isdef & f_i(\struc(\acomp_i)) \text{, for all $i \in \interv{1}{\ncomps}$} \\
\hspace*{-2mm}(\vec{f}(\struc))(\ainterac_j) & \isdef & \{\tuple{f_{i_1}(u_1), \ldots, f_{i_{\#(\ainterac_j)}}(u_{\#(\ainterac_j)})} \mid
  \tuple{u_1, \ldots, u_{\#(\ainterac_j)}} \in \struc(\ainterac_j),~ \\
&& \hspace*{4cm} \forall \ell \in \interv{1}{\#(\ainterac_j)} ~.~ \compof{\tuple{\portsof{\ainterac_j}}_\ell} = \acomp_{i_\ell}\}
\end{array}\]
If, moreover, $\amark$ is a marking of the Petri net
$\anetof{\signature,\struc,\beh}$, we define $\vec{f}(\amark) \isdef
\set{q[f_i(u)] \mid q[u] \in \amark,~ q \in \statesof{\acomp_i},~ i
  \in \interv{1}{\ncomps}}$; since the sets $\statesof{\acomp_i}$, for
$i \in \interv{1}{\ncomps}$, have been assumed to be pairwise
disjoint, there is exactly one component type $\acomp_i$, such that $q
\in \statesof{\acomp_i}$. Two configurations $(\struc_i,\amark_i)$,
for $i = 1,2$ are \emph{isomorphic}, denoted $(\struc_1,\amark_1)
\symm{} (\struc_2,\amark_2)$, if and only if there exists a tuple of
bijections $\vec{f} = \tuple{f_1, \ldots, f_\ncomps}$, such that
$\vec{f}(\struc_1) = \struc_2$ and $\vec{f}(\amark_1) =
\amark_2$. First, we show that the \adl\ logic cannot distinguish
isomorphic configurations:

\begin{lemma}\label{lemma:isomorphism-indistinguishability}
  Given configurations $(\struc_i,\amark_i)$, for $i=1,2$, such that
  $(\struc_1,\amark_1) \symm{} (\struc_2,\amark_2)$, for any sentence
  $\phi$, we have $(\struc_1,\amark_1) \models \phi \iff
  (\struc_2,\amark_2) \models \phi$. 
\end{lemma}
\proof{ Let $\vec{f} = \tuple{f_1, \ldots, f_\ncomps}$ be a tuple of
  bijections. We prove the more general statement $(\struc,\amark)
  \models^\store \phi \iff (\vec{f}(\struc),\vec{f}(\amark))
  \models^{f \circ \store} \phi$, for any configuration
  $(\struc,\amark)$ and any formula $\phi$, by induction on the
  definition of the satisfaction relation $\models^\store$,
  distinguishing the following cases: \begin{itemize}
    %
  \item $\phi = \emp$: $\struc(\acomp_i) = \emptyset \iff
    (\vec{f}(\struc))(\acomp_i) = (f_i(\struc))(\acomp_i) =
    \emptyset$, for $i \in \interv{1}{\ncomps}$, $\struc(\ainterac_j)
    = \emptyset \iff (\vec{f}(\struc))(\ainterac_j) = \emptyset$, for
    $j \in \interv{1}{\ninteracs}$ and $\amark = \emptyset \iff
    \vec{f}(\amark) = \emptyset$.
    %
  \item $\phi = \acomp_i(x)$: $\struc(\acomp_i) = \set{\store(x)} \iff 
  \end{itemize} \qed}

Given a function $f : \universe \rightarrow \universe$ and an
architecture $\struc$, we denote by $f(\struc)$ the
architecture: \begin{compactitem}
  %
\item $(f(\struc))(\acomp_i) = f(\struc(\acomp_i))$, for all $i \in
  \interv{1}{\ncomps}$,
  %
\item $(f(\struc))(\ainterac_j) = f(\struc(\ainterac_j))$, for all $j
  \in \interv{1}{\ninteracs}$,
  %
\end{compactitem}
where $f$ is naturally lifted to sets, tuples and sets of
tuples. Moreover, for a marking $\amark$ of a Petri net, we denote by
$f(\amark)$ the set $\set{q[f(u)] \mid q[u] \in \amark}$. Below we
show that the semantics of \adl\ formul{\ae}, as well as the sets of
reachable and deadlock markings of a Petri net defined by a structure
are closed under permutations of its indices.

\begin{lemma}\label{lemma:permutation-closure}
  Given an architecture $\struc$ and a behavior $\beh$, over a
  signature $\signature$, for any bijection $f : \universe \rightarrow
  \universe$, the following hold: \begin{enumerate}
    %
  \item\label{it1:permutation-closure} $(\struc,\amark) \models \phi
    \iff (f(\struc),f(\amark)) \models \phi$, for any sentence $\phi$, 
    %
  \item\label{it2:permutation-closure} $\amark \in
    \step{\anetof{\signature,\struc,\beh},\amark_0} \iff f(\amark) \in
    \step{\anetof{\signature,f(\struc),\beh}, f(\amark_0)}$,
    %
  \item\label{it3:permutation-closure} $\amark \in
    \reach{\anetof{\signature,\struc,\beh}, \amark_0} \iff f(\amark)
    \in \reach{\anetof{\signature, f(\struc), \beh}, f(\amark_0)}$,
    %
  \item\label{it4:permutation-closure} $\amark \in
    \dead{\anetof{\signature,\struc,\beh}} \iff f(\amark) \in
    \dead{\anetof{\signature,f(\struc),\beh}}$,
    %
  \end{enumerate}
  for any two markings $\amark_0,\amark$ of
  $\anetof{\signature,\struc,\beh}$.
\end{lemma}
\proof{ (\ref{it1:permutation-closure}) We prove the more general
  statement $(\struc,\amark) \models^\store \phi \iff
  (f(\struc),f(\amark)) \models^{f \circ \store} \phi$, for any
  formula $\phi$, by induction on the definition of the satisfaction
  relation $\models^\store$, distinguishing the following
  cases: \begin{itemize}
    %
  \item $\phi = \emp$: $\struc(\acomp) = \emptyset \iff
    (f(\struc))(\acomp) = \emptyset$, for all $\acomp \in \comps$ and
    $\struc(\ainterac) = \emptyset \iff (f(\struc))(\ainterac) =
    \emptyset$, for all $\ainterac \in \interacs$.
    %
  \item $\phi = \acomp(x)$: $\struc(\acomp) = \set{\store(x)} \iff
    (f(\struc)))(\acomp) = \set{f(\store(x))}$, $\struc(\acomp') =
    \emptyset \iff (f(\struc))(\acomp') = \emptyset$, for all $\acomp'
    \in \comps \setminus \set{\acomp}$ and $\struc(\ainterac) =
    \emptyset \iff (f(\struc))(\ainterac) = \emptyset$, for all
    $\ainterac\in\interacs$.
    %
  \item $\phi = \ainterac(x_1, \ldots, x_{\#(\ainterac)})$:
    $\struc(\ainterac) = \set{\tuple{\store(x_1), \ldots,
      \store(x_{\#(\ainterac)})}} \iff (f(\struc))(\ainterac) =
    \set{\tuple{f(\store(x_1)), \ldots,
        f(\store(x_{\#(\ainterac)}))}}$, $\struc(\acomp) = \emptyset
    \iff (f(\struc))(\acomp) = \emptyset$, for all $\acomp \in \comps$
    and $\struc(\ainterac') = \emptyset \iff (f(\struc))(\ainterac') =
    \emptyset$, for all $\ainterac' \in \interacs \setminus
    \set{\ainterac}$.
    %
  \item $\phi = \phi_1 * \phi_2$: by an application of the inductive
    hypothesis, using the equivalence $(f(\struc),f(\amark)) =
    (f(\struc_1),f(\amark_1)) \comp (f(\struc_2),f(\amark_2)) \iff
    (\struc,\amark) = (\struc_1,\amark_1) \comp (\struc_2,\amark_2)$.
    %
  \item $\phi \in \set{\apred(x_1,\ldots,x_{\#(\apred)}), \phi_1 \vee
    \phi_2, \exists x ~.~ \phi_1}$: by an application of the inductive
    hypothesis.
  \end{itemize}

  \vspace*{\baselineskip} \noindent (\ref{it2:permutation-closure}),
  (\ref{it3:permutation-closure}), (\ref{it4:permutation-closure}): by
  Def. \ref{def:execution-semantics}, let
  $\anetof{\signature,f(\struc),\beh}$ be the Petri net $(\places^f,
  \trans^f, \edges^f)$, where: 
  \[\begin{array}{rcl}
  \places^f & = & \bigcup_{\acomp\in\comps} \set{q[u] \mid q
    \in \compstates{\acomp},~ u \in (f(\struc))(\acomp)} \\
  & = & \bigcup_{\acomp\in\comps} \set{q[f(u)] \mid q \in
    \compstates{\acomp},~ u \in \struc(\acomp)}
  \\[2mm]
  \trans^f & = & \bigcup_{\ainterac\in\interacs}
  \{ ~ (\ainterac[u_1,\ldots,u_{\#(\ainterac)}], \tuple{t_1,\ldots, t_{\#(\ainterac)}})
  ~\mid~ \\[1mm]
  & & \hspace{1.5cm} \tuple{u_1,\ldots,u_{\#(\ainterac)}} \in (f(\struc))(\ainterac),~
  \tuple{p_1, \ldots, p_{\#(\ainterac)}} = \interportsof{\ainterac}, \\[1mm]
  & & \hspace{1.5cm} \forall i \in \interv{1}{\#(\ainterac)}.~ t_i = (q \arrow{p_i}{} q') \in \arrow{}{\compof{p_i}}  \\[1mm]
  & & \hspace{1.5cm} \forall i,j \in \interv{1}{\#(\ainterac)}.~ i\not=j \Rightarrow
  u_i\not=u_j \mbox{ or } \compof{p_i} \not= \compof{p_j} ~ \} \\
  & = & \bigcup_{\ainterac\in\interacs}
  \{ ~ (\ainterac[f(u_1),\ldots,f(u_{\#(\ainterac)})], \tuple{t_1,\ldots, t_{\#(\ainterac)}})
  ~\mid~ \\[1mm]
  & & \hspace{1.5cm}
  \tuple{u_1,\ldots,u_{\#(\ainterac)}} \in \struc(\ainterac),~
  \tuple{p_1, \ldots, p_{\#(\ainterac)}} = \interportsof{\ainterac}, \\[1mm]
  & & \hspace{1.5cm} \forall i \in \interv{1}{\#(\ainterac)}.~ t_i = (q \arrow{p_i}{} q') \in \arrow{}{\compof{p_i}}  \\[1mm]
  & & \hspace{1.5cm} \forall i,j \in \interv{1}{\#(\ainterac)}.~ i\not=j \Rightarrow
  u_i\not=u_j \mbox{ or } \compof{p_i} \not= \compof{p_j} ~ \}
  \end{array}\]
  \[\begin{array}{rcl}
  \edges^f & = & \bigcup_{\ainterac\in\interacs}
  \{ ~ (q[f(u_i)], (\ainterac[f(u_1),\ldots,f(u_{\#(\ainterac)})], \tuple{t_1,\ldots, t_{\#(\ainterac)}}) ), \\[1mm]
  & & \hspace{1cm} ((\ainterac[f(u_1),\ldots,f(u_{\#(\ainterac)})], \tuple{t_1,\ldots, t_{\#(\ainterac)}}), q'[f(u_i)]) ~\mid ~\\[1mm]
  & & \hspace{1.5cm} t_i = (q \arrow{p_i}{} q'),~i \in \interv{1}{\#(\ainterac)} ~ \}
  \end{array}\]
  We obtain the following equivalence: \[\begin{array}{c}
  \amark \arrow{(\ainterac[u_1, \ldots,
      u_{\#(\ainterac)}], \tuple{t_1, \ldots, t_{\#(\ainterac)}})}{}
  \amark' \text{ in $\anetof{\signature,\struc,\beh}$} \\
  \iff \\
  f(\amark) \arrow{(\ainterac[f(u_1), \ldots,
      f(u_{\#(\ainterac)})], \tuple{t_1, \ldots,
      t_{\#(\ainterac)}})}{} f(\amark') \text{ in
    $\anetof{\signature,f(\struc),\beh}$}
  \end{array}\] Point
  (\ref{it2:permutation-closure}) uses this argument directly. Point
  (\ref{it3:permutation-closure}) applies this argument inductively,
  on the length of the firing sequence. For point
  (\ref{it4:permutation-closure}), we use, moreover, that $q[u] \in
  \amark \iff q[f(u)] \in f(\amark)$ and $q[u] \in
  \pre{(\ainterac[u_1, \ldots, u_{\#(\ainterac)}],\tuple{t_1, \ldots,
      t_{\#(\ainterac)}})} \iff q[f(u)] \in \pre{(\ainterac[f(u_1),
      \ldots, f(u_{\#(\ainterac)})],\tuple{t_1, \ldots,
      t_{\#(\ainterac)}})}$. \qed}

Symmetry is defined as an equivalence relation between configurations:
\begin{definition}\label{def:symmetry-relation}
  Given configurations $(\struc_1, \amark_1)$ and $(\struc_2,
  \amark_2)$, we define the relation $(\struc_1,\amark_1) \symm{}
  (\struc_2,\amark_2)$ if and only if there exists a bijection $f :
  \universe \rightarrow \universe$, such that $f(\struc_1) = \struc_2$
  and $f(\amark_1) = \amark_2$.
\end{definition}
Given a sentence $\phi$, we assume, for each model $(\struc,\amark)$
of $\phi$, the existence of a bijection $\canon : \universe
\rightarrow \universe$, such that $(\canon(\struc), \canon(\amark))$
is a (not necessarily canonical) representative of the model's
equivalence class (w.r.t. $\symm{}$) and let $\csem{\phi}{\asid}$ denote
the set of representatives of the models of $\phi$, interpreted over a
given SID $\asid$. The main result of this section states the
equivalence between the original decision problems, where every model
of a sentence is considered and the versions in which only the
representatives of the equivalence classes with respect to the $\symm{}$
relation (Def. \ref{def:symmetry-relation}) are considered:

\begin{theorem}\label{thm:symmetry}
  Given sentences $\phi$ and $\psi$, interpreted over a SID $\asid$,
  and a behavior $\beh$, the following equivalences hold: 
  \[\begin{array}{rcl}
  \mathit{deadlock}^\canon(\phi,\asid,\beh) & \iff & \mathit{deadlock}(\phi,\asid,\beh) \\
  \mathit{reach}^\canon(\phi,\psi,\asid,\beh) & \iff & \mathit{reach}(\phi,\psi,\asid,\beh) \\
  \mathit{safe}^\canon(\phi,\psi,\asid,\beh) & \iff & \mathit{safe}(\phi,\psi,\asid,\beh) \\
  \mathit{inductive}^\canon(\phi,\asid,\beh) & \iff & \mathit{inductive}(\phi,\asid,\beh)
  \end{array}\]
  where the queries $\mathit{deadlock}^\canon(\phi,\asid,\beh)$,
  $\mathit{reach}^\canon(\phi,\psi,\asid,\beh)$,
  $\mathit{safe}^\canon(\phi,\psi,\asid,\beh)$ and
  $\mathit{inductive}^\canon(\phi,\asid,\beh)$ are defined
  below: \begin{itemize}
  %
\item $\mathit{deadlock}^\canon(\phi,\asid,\beh)$: is there a configuration
  $(\struc,\amark) \in \csem{\phi}{\asid}$, such that
  $\reach{\anetof{\signature,\struc,\beh},\amark} \cap
  \dead{\anetof{\signature,\struc,\beh}} \neq \emptyset$ ?
  %
\item $\mathit{reach}(\phi,\psi,\asid,\beh)$: are there configurations
  $(\struc,\amark) \in \csem{\phi}{\asid}$ and $(\struc,\amark') \in
  \csem{\phi}{\asid}$, such that $\amark' \in
  \reach{\anetof{\signature,\struc,\beh},\amark}$ ?
  %
\item $\mathit{safe}(\phi,\psi,\asid,\beh)$: for each configuration
  $(\struc,\amark) \in \csem{\phi}{\asid}$ and each marking $\amark'
  \in \reach{\anetof{\signature,\struc,\beh},\amark}$, is it true that
  $(\struc,\amark') \in \csem{\psi}{\asid}$ ?
  %
\item $\mathit{inductive}(\phi,\asid,\beh)$: for each configuration
  $(\struc,\amark) \in \csem{\phi}{\asid}$ and each marking $\amark'
  \in \step{\anetof{\signature,\struc,\beh},\amark}$, is it true that
  $(\struc,\amark') \in \csem{\phi}{\asid}$ ?
  \end{itemize}  
\end{theorem}
\proof{
  We prove the following points:

  \vspace*{\baselineskip}
  \noindent$\mathit{deadlock}(\phi,\asid,\beh) \iff
  \mathit{deadlock}^{\canon}(\phi,\asid,\beh)$: ``$\Rightarrow$'' Let
  $(\struc,\amark)\in\sem{\phi}{\asid}$ and $\amark' \in
  \reach{\anetof{\signature,\struc,\beh},\amark} \cap
  \dead{\anetof{\signature,\struc,\beh}}$. Then $(\canon(\struc),
    \canon(\amark)) \in \csem{\phi}{\asid}$, where $\canon$ is a
    bijection that maps $(\struc,\amark)$ into a representative of its
    equivalence class w.r.t. $\symm{}$. By points
    \ref{it3:permutation-closure} and \ref{it4:permutation-closure} of
    Lemma \ref{lemma:permutation-closure}, we obtain that
    $\canon(\amark') \in
    \reach{\anetof{\signature,\canon(\struc),\beh},\canon(\amark)}
    \cap
    \dead{\anetof{\signature,\canon(\struc),\beh}}$. ``$\Leftarrow$''
    Because $\csem{\phi}{\asid} \subseteq \sem{\phi}{\asid}$.

  \vspace*{\baselineskip}
  \noindent$\mathit{reach}(\phi,\psi,\asid,\beh) \iff
  \mathit{reach}^{\canon}(\phi,\psi,\asid,\beh)$: ``$\Rightarrow$''
  Let $(\struc,\amark)\in\sem{\phi}{\asid}$ and $\amark' \in
  \reach{\anetof{\signature,\struc,\beh},\amark} \cap
  \sem{\psi}{\asid}$. Then $(\canon(\struc), \canon(\amark)) \in
  \csem{\phi}{\asid}$, where $\canon$ is a bijection that maps
  $(\struc,\amark)$ into a representative of its equivalence class
  w.r.t. $\symm{}$. By points \ref{it1:permutation-closure} and
  \ref{it3:permutation-closure} of Lemma
  \ref{lemma:permutation-closure}, we obtain that $\canon(\amark') \in
  \reach{\anetof{\signature,\canon(\struc),\beh},\canon(\amark)} \cap
  \csem{\psi}{\asid}$. ``$\Leftarrow$'' Because $\csem{\phi}{\asid}
  \subseteq \sem{\phi}{\asid}$ and $\csem{\psi}{\asid} \subseteq
  \sem{\psi}{\asid}$.

  \vspace*{\baselineskip}
  \noindent$\mathit{safe}(\phi,\psi,\asid,\beh) \iff
  \mathit{safe}^{\canon}(\phi,\psi,\asid,\beh)$: ``$\Rightarrow$'' Let
  $(\struc,\amark) \in \csem{\phi}{\asid}$ and $\amark' \in
  \reach{\anetof{\signature,\struc,\beh},\amark}$. Then
  $(\struc,\amark)$ is a representative of a configuration
  $(\canon^{-1}(\struc), \canon^{-1}(\amark)) \in \sem{\phi}{\asid}$,
  where $\canon$ is a bijection mapping that configuration into
  $(\struc,\amark)$. By point \ref{it3:permutation-closure} of Lemma
  \ref{lemma:permutation-closure}, we obtain $\canon^{-1}(\amark') \in
  \reach{\anetof{\signature,\canon^{-1}(\struc),\beh},\canon^{-1}(\amark)}$,
  thus $(\canon^{-1}(\struc), \canon^{-1}(\amark')) \in
  \sem{\psi}{\asid}$, leading to $(\struc,\amark') \in
  \csem{\psi}{\asid}$. ``$\Leftarrow$'' Let $(\struc,\amark) \in
  \sem{\phi}{\asid}$ and $\amark' \in
  \reach{\anetof{\signature,\struc,\beh},\amark}$. Let $\canon$ be a
  bijection that maps $(\struc,\amark)$ into a representative, leading
  to $(\canon(\struc), \canon(\amark)) \in \csem{\phi}{\asid}$. By
  point \ref{it3:permutation-closure} of Lemma
  \ref{lemma:permutation-closure}, we obtain $\canon(\amark') \in
  \reach{\anetof{\signature,\canon(\struc),\beh}, \canon(\amark)}$,
  thus $(\canon{\struc}, \canon{\amark'}) \in \csem{\psi}{\asid}$,
  leading to $(\struc,\amark') \in \sem{\psi}{\asid}$.

  \vspace*{\baselineskip}
  \noindent$\mathit{inductive}(\phi,\asid,\beh)\iff\mathit{inductive}^{\canon}(\phi,\asid,\beh)$:
  using a similar reasoning as above, relying on point
  \ref{it4:permutation-closure} of Lemma
  \ref{lemma:permutation-closure}.
  \qed}

